P3: Prompts Promote Prompting

Current large language model (LLM) applications often employ multi-component prompts, comprising both system and user prompts, to guide model behaviors. While recent advancements have demonstrated the efficacy of automatically optimizing either the system or user prompt to boost performance, such unilateral approaches often yield suboptimal outcomes due to the interdependent nature of these components. In this work, we introduce P3, a novel self-improvement framework that concurrently optimizes both system and user prompts through an iterative process. The offline optimized prompts are further leveraged to promote online prompting by performing query-dependent prompt optimization. Extensive experiments on general tasks (e.g., Arena-hard and Alpaca-eval) and reasoning tasks (e.g., GSM8K and GPQA) demonstrate that P3 achieves superior performance in the realm of automatic prompt optimization. Our results highlight the effectiveness of a holistic optimization strategy in enhancing LLM performance across diverse domains.

==> data/method_old.tex <==
\section{Methodology}

In this section, we introduce the background and overall framework of P3. We first give the task formulation for automatic prompt optimization in section ~\ref{sec:task}. Then we describe the algorithm details of P3 in section~\ref{sec:p3}.

\subsection{Task Definition}
\label{sec:task}
In this work, we focus on black-box prompt optimization~\citep{BPO,PAS}, which can be formulated as a discrete optimization problem:
\begin{equation}
    x^* = \arg\max_{x\in\mathcal{X}}P(y|llm(x))
\end{equation}
where $x$ is the input prompt, which contain both the system part and user part. $x^*$ is the the optimal prompt that best suit the $llm(.)$ to answer, which means to maximize the probability to generate the ground truth $y$ based on the input prompt $x$. Current prompt logically divided into two parts: the system prompt $x_s$, which defines the role, capability or other global constrains for LLM to follow, and the user prompt $x_u$, which gives the concrete requirements for current conversation. However, previous methods mostly focus on either system prompt or user prompt optimization, while keeping the other part unchanged:
\begin{equation}
\label{eq:sys_opt}
    (x_s, x_u^*) = \arg\max_{x_u\in\mathcal{X}_u}P(y | llm(x_s, x_u))
\end{equation}
\begin{equation}
\label{eq:usr_opt}
    (x_s^*, x_u) = \arg\max_{x_s\in\mathcal{X}_s}P(y | llm(x_s, x_u))
\end{equation}

which results in a sub-optimal prompt and answer. To alleviate this problem, we propose the Prompts Promote Prompting~(P3) to joint optimize the system and user prompts.


\subsection{Prompts Promote Prompting}
\label{sec:p3}
Figure \ref{fig:methods} shows the main process of P3. Since the system prompt is always consistent in a certain scenario, while user prompt differs case by case. Thus, we adopt different optimization strategies for system and user prompts. Following is the detail descriptions for the whole offline optimization and online prediction 





\subsubsection{User Prompt Optimization}
\label{sec:usr}

In each call to an agent, the user prompt may differs a lot, thus the user prompt optimization should conduct online. However, the strict constrains for online prediction latency making it unlikely to perform complex optimization algorithm. Thus, we convert the online process into an mapping: $\mathcal{F}: x_u \rightarrow x_u^*$, 
which can be conducted through a feed forward small language model~\citep{PAS}. 
procedures.

Therefore, the objective for offline user prompt optimization can be represented as:
\begin{equation}
    \mathcal{J}= \max_{x_u\in X_u} P(x_u^* | f(x_u))   
\end{equation}
As the ground truth user prompt $x_u^*$ is inaccessible in most situation, so we propose the user prompt optimization methods for offline data construction. As shown in Algorithm~\ref{alg1}, we first generate K candidate user prompt expansions via LLM. Then, the candidate expansion are concatenated with the system prompt to generate the answers. And we score each answer via LLM as judge. Then the expansions and scores are fed into an iterative optimization loop in Algorithm~\ref{alg1} with system prompt optimization in \ref{sec:sys}. Finally, we collect the dataset of user prompt and its corresponding optimized user prompt for model training shown in section~\ref{sec:train}. 




\subsubsection{System Prompt Optimization}
\label{sec:sys}
For system prompt optimization, the objective is to learn a prompt $x_s$ that generalize to the user prompts best as shown in Eq.\ref{eq:sys_opt}. However, the optimization process occurs several challenges in practical conditions. First, the ground truth $y$ is also inaccessible, resulting in difficult in evaluating the system prompt performance. Second, the parameter space of system prompt fall into the whole text sequence space, which is infinite theoretically. Based on the above situation, we follow the discrete optimization methods\cite{opro}, and propose the system prompt optimization methods show in Fig.~\ref{fig:methods}(b). Specifically, as shown in Algorithm~\ref{alg:sys}, we first initialize a group of system prompt $X_s$ based on the raw system prompt $x_s$ via LLM generation. Then, the system prompts group will catenate with the user prompt to form the complete prompts and obtain the final answers through LLM. Later, we adopt LLM as an evaluator to score the answers corresponding to the system prompt group and filter out the top-k system prompts. Then, we use the top-k system prompts as few-shot samples to generate a new group of $X_s$. Finally, we evaluate $X_s$ as above and return the best system prompt to the next iteration of user prompt optimization. 



\subsubsection{Online Prediction}
After obtaining the optimized system prompt and the user prompt expansion model, the online prediction process can be represented as:
\begin{equation}
    y=LLM(x_s^*, f_\theta(x_u))
\end{equation}
where $f_\theta(.)$ is the trained small language model in section~\ref{sec:train} that expand the user prompt $x_u$ to $x_u^*$. Then $x_u^*$ is concatenated with the optimized system prompt $x_s^*$ described in section~\ref{sec:sys} to generate the final response $y$. 


\subsubsection{Model Training}
\label{sec:train}
After collecting the ground truth of user prompt expansions from section~\ref{sec:usr}, we train a small language model to fit the user prompt optimization loss:
\begin{equation}
    \mathcal{L}_{x_u}(\theta) = \sum_{x_u\in X_u}-P(x_u^*|f(x_u;\theta))
\end{equation}
